Linear stability analysis of wall-bounded high-pressure transcritical fluids

Mixing and heat transfer rates are typically enhanced when operating at high-pressure transcritical turbulent flow regimes. The rapid variation of thermophysical properties in the vicinity of the pseudo-boiling region can be leveraged to significantly increase the Reynolds numbers and destabilize the flow. The underlying physical mechanism responsible for this destabilization is the presence of a baroclinic torque mainly driven by large localized density gradients across the pseudo-boiling line. As a result, the enstrophy levels are enhanced compared to equivalent low-pressure cases, and the flow physics behavior deviates from standard wall turbulence characteristics. In this work, the nature of this instability is carefully analyzed and characterized by means of linear stability theory. It is found that, at isothermal wall-bounded transcritical conditions, the non-linear thermodynamics exhibited near the pseudo-boiling region propitiates the laminar-to-turbulent transition with respect to sub- and super-critical thermodynamic states. This transition is further exacerbated for non-isothermal flows even at low Brinkman numbers. Particularly, neutral curve sensitivity to Brinkman numbers and perturbation profiles of dynamic and thermodynamic unstable modes based on modal and non-modal analysis, which trigger the early flow destabilization, confirm this phenomenon. Nonetheless, a non-isothermal setup is a necessary condition for transition when operating at low-Mach/Reynolds-number regimes. In detail, on equal Brinkman number, turbulence transition is accelerated and algebraic growth enhanced in comparison to isothermal cases. Consequently, high-pressure transcritical setups result in larger kinetic energy budgets due to larger production rates and lower viscous dissipation.

==> jfm_bib <==
% This is jfm2esam.bib v1.0 08/14/02
%

@InBook{AbramowitzStegun1970,
 author = {M. Abramowitz and I. Stegun},
 title = {Handbook of Mathematical Functions},
 publisher = {Dover},
 edition = {9},
 pages = {3.3.7},
 year = {1970}
 }

 @Article{BarkerSchaefferBohorquezGray2015,
 author      = {T. Barker and D. G. Schaeffer and P. Boh\'orquez and J. M. N. T. Gray},
 title       = {Well-posed and ill-posed behaviour of the $\mu(\protect{I})$-rheology for granular flows},
 journal     = {J. Fluid. Mech.},
 year        = {2015},
 volume      = {779},
 pages       = {794--818}

 }

@Article{Batchelor59,
  author = 	 {G.K. Batchelor},
  title = 	 {Small-scale variation of convected quantities like temperature in turbulent fluid Part 1. General discussion and the case of small conductivity.},
  journal = 	 {J. Fluid Mech.},
  year = 	 {1971},
  volume = 	 {5},
  pages = 	 {113--133}
}

@inproceedings{Briukhanovetal1967,
 author      = {A. V. Briukhanov and S. S. Grigorian and S. M. Miagkov and M. Y. Plam and I. E. Shurova and M. E. Eglit and Y. L. Yakimov},
 title       = {On some new approaches to the dynamics of snow avalanches},
 booktitle   = {Physics of Snow and Ice,  Proceedings of the International Conference on Low Temperature Science},
 volume      = {1},
 number      = {2},
 pages       = {1221--1241},
 publisher   = {Institute of Low Temperature Science, Hokkaido University, Sapporo, Hokkaido, Japan},
 year        = {1967}
 }

@Article{Brownell04,
  author = 	 {C.J. Brownell and L.K. Su},
  title = 	 {Planar measurements of differential diffusion in turbulent jets},
  journal = 	 {AIAA Paper 2004-2335},
  year = {2004}
}

@Article{Brownell07,
  author = 	 {C.J. Brownell and L.K. Su},
  title = 	 {Scale relations and spatial spectra in a differentially diffusing jet},
  journal = 	 {AIAA Paper 2007-1314},
  year = {2007}
  }

@InCollection{Dennis85,
  author = 	 {S.C.R. Dennis},
  title = 	 {{Compact explicit finite difference approximations to the Navier--Stokes equation}},
  booktitle = 	 {Ninth Intl Conf. on Numerical Methods in Fluid Dynamics},
  publisher = {Springer},
  year = 	 {1985},
  editor = 	 {Soubbaramayer and J.P. Boujot},
  volume = 	 {218},
  series = 	 {Lecture Notes in Physics},
  pages = 	 {23--51},
}

@Article{EdwardsVirouletKokelaarGray2017,
	title    = {Formation of levees, troughs and elevated channels by avalanches on erodible slopes},
	author   = {Edwards, A. N. and Viroulet, S. and Kokelaar, B. P. and Gray, J. M. N. T.},
	journal  = {J. Fluid Mech.},
	volume   = {823},
	pages    = {278--315},
	year     = {2017}
}

@Article{Hwang70,
  author = 	 {L.-S. Hwang and E.O. Tuck},
  title = 	 {On the oscillations of harbours of arbitrary shape},
  journal = 	 {J.~Fluid Mech.},
  year = 	 {1970},
  volume = 	 {42},
  pages = 	 {447--464},
}

@Article {JosephSaut1990,
 author= {Joseph, Daniel D. and Saut, Jean Claude},
 title = {Short-wave instabilities and ill-posed initial-value problems},
 journal = {Theoretical and Computational Fluid Dynamics},
 publisher= {Springer Berlin / Heidelberg},
 issn= {0935-4964},
 keyword= {Physics and Astronomy},
 pages = {191--227},
 volume  = {1},
 issue = {4},
 howpublished = {\url{http://dx.doi.org/10.1007/BF00418002}},
 note = {10.1007/BF00418002},
 year = {1990}
 }

@InCollection{Worster92,
  author = 	 {M.G. Worster},
  title = 	 {{The dynamics of mushy layers}},
  booktitle = 	 {Interactive dynamics of convection and solidification},
  publisher = {Kluwer},
  year = 	 {1992},
  editor = 	 {S.H. Davis and H.E. Huppert and W. Muller and M.G. Worster},
  pages = 	 {113--138},
}

@Article{Koch83,
  author = 	 {W. Koch},
  title = 	 {Resonant acoustic frequencies of flat plate cascades},
  journal = 	 {J.~Sound Vib.},
  year = 	 {1983},
  volume = 	 {88},
  pages = 	 {233--242},
}

@Article{Lee71,
  author = 	 {J.-J. Lee},
  title = 	 {Wave-induced oscillations in harbours of arbitrary geometry},
  journal = 	 {J.~Fluid Mech.},
  year = 	 {1971},
  volume = 	 {45},
  pages = 	 {375--394},
}

@Article{Linton92,
  author = 	 {C.M. Linton and D.V. Evans},
  title = 	 {The radiation and scattering of surface waves by a vertical circular
cylinder in a channel},
  journal = 	 {Phil.\ Trans.\ R. Soc.\ Lond.},
  year = 	 {1992},
  volume = 	 {338},
  pages = 	 {325--357},
}

@Article{Martin80,
  author = {P.A. Martin},
  title =  {On the null-field equations for the exterior problems of acoustics},
  year ={1980},
  journal = {Q.~J. Mech.\ Appl.\ Maths},
  volume = {33},
  pages ={385--396},
}

@TechReport{Rogallo81,
   author = {R.S. Rogallo},
   title = {Numerical experiments in homogeneous
     turbulence},
   institution = {NASA Tech.\ Mem.},
   year = 1981,
   number = 81835
}

@Article{Ursell50,
  author = {F. Ursell},
  title = {Surface waves on deep water in the presence of a submerged cylinder I},
  year = {1950},
  journal = {Proc.\ Camb.\ Phil.\ Soc.},
  volume = {46},
  pages = {141--152}
}

@Article{Wijngaarden68,
  author = {L. {van Wijngaarden}},
  title = {On the oscillations Near and at resonance in open pipes},
  year = {1968},
  journal = {J.~Engng Maths},
  volume = {2},
  pages = {225--240}
}

@PhdThesis{Miller91,
  author = {P.L. Miller},
  title = {Mixing in high Schmidt number turbulent jets},
  school = {California Institute of Technology},
  year = {1991},
  address = {}
}

@electronic{Bouguet01,
author={Bouguet, J.-Y},
year={2008},
  title = {Camera Calibration Toolbox for Matlab},
 howpublished = {\url{http://www.vision.caltech.edu/bouguetj/calib_doc/}}
}


%% End of file `jfm2esam.bib'.

